LOPR: Latent Occupancy PRediction using Generative Models

Environment prediction frameworks are integral for autonomous vehicles, enabling safe navigation in dynamic environments. LiDAR generated occupancy grid maps (L-OGMs) offer a robust bird's eye-view scene representation that facilitates joint scene predictions without relying on manual labeling unlike commonly used trajectory prediction frameworks. Prior approaches have optimized deterministic L-OGM prediction architectures directly in grid cell space. While these methods have achieved some degree of success in prediction, they occasionally grapple with unrealistic and incorrect predictions. We claim that the quality and realism of the forecasted occupancy grids can be enhanced with the use of generative models. We propose a framework that decouples occupancy prediction into: representation learning and stochastic prediction within the learned latent space. Our approach allows for conditioning the model on other available sensor modalities such as RGB-cameras and high definition maps. We demonstrate that our approach achieves state-of-the-art performance and is readily transferable between different robotic platforms on the real-world NuScenes, Waymo Open, and a custom dataset we collected on an experimental vehicle platform.

==> Figures/datasets.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[height=3cm, width=13cm]{example-image-a}
    \caption{Example of preprocessed samples from NuScenes, Waymo Open Perception, and our custom datasets.}
    \label{fig:datasets}
\end{figure}

==> Figures/prediction.tex <==

\begin{figure} 
  \centering
  \input{Figures/prediction-2}
  \vspace{0.1cm}
  \input{Figures/prediction-1}
  \vspace{0.1cm}
  \input{Figures/prediction-3}
\caption{Example predictions from NuScenes, Waymo Open Perception, and Custom Robotic datasets (ordered from top to bottom). We visualize the best sample out of 50, and a random one. Ego vehicle is in the center moving to the right. From the top: 1) Oncoming vehicle is passing our ego to the left of it. Our stochastic model is capable of hallucinating a vehicle entering the observable part of the OGM. 2) Ego vehicle is surrounded by traffic. 3) Ego vehicle is passed by a large bus. In all of the scenarios, LOPR correctly propagates the moving objects. }
\label{fig:prediction}
\end{figure}

==> Tables/inference_time.tex <==
\begin{table}[h]
\caption{Comparison of the training time.}
\small
      \centering
        \begin{tabular}{@{}lrr@{}} \toprule
        \textbf{Model}  & \textbf{Training Time} & \textbf{Inference Time} \\ \midrule
        LOPR &   \\
        Representation Learning with VAE-GAN & 140 hrs 29 mins &\\ 
        Representation Learning with VAE & 39 hrs 58 mins & \\ 
        Supervised Learning & approx. 10 mins & \\ \midrule
        PredNet with TAAConvLSTM & 51 hrs 52 mins & \\
        PredNet with ConvLSTM & 24 hrs 59 mins & \\
        DVG & 128 hrs 35 mins & \\
        SRVP & 107 hrs 37 mins & \\ \midrule 
        \end{tabular}
    \label{table:trainig_time}
    \vspace{-2.5em}
\end{table} 

